Search for an excess of events in the Super-Kamiokande detector in the directions of the astrophysical neutrinos reported by the IceCube Collaboration

We present the results of a search in the Super-Kamiokande (SK) detector for excesses of neutrinos with energies above a few GeV that are in the direction of the track events reported in IceCube. Data from all SK phases (SK-I through SK-IV) were used, spanning a period from April 1996 to April 2016 and corresponding to an exposure of 225 kilotonne-years . We considered the 14 IceCube track events from a data set with 1347 livetime days taken from 2010 to 2014. We use Poisson counting to determine if there is an excess of neutrinos detected in SK in a 10 degree search cone (5 degrees for the highest energy data set) around the reconstructed direction of the IceCube event. No significant excess was found in any of the search directions we examined. We also looked for coincidences with a recently reported IceCube multiplet event. No events were detected within a $\pm$ 500 s time window around the first detected event, and no significant excess was seen from that direction over the lifetime of SK.

==> authors_arXiv.tex <==
K. Abe, C. Bronner, G. Pronost, Y. Hayato, M. Ikeda, K. Iyogi, J. Kameda, Y. Kato, Y. Kishimoto, Ll. Marti, M. Miura, S. Moriyama, M. Nakahata, Y. Nakano, S. Nakayama, Y. Okajima, A. Orii, H. Sekiya, M. Shiozawa, Y. Sonoda, A. Takeda, A. Takenaka, H. Tanaka, S. Tasaka, T. Tomura, R. Akutsu, T. Kajita, K. Kaneyuki, Y. Nishimura, K. Okumura, K. M. Tsui, L. Labarga, P. Fernandez, F. d. M. Blaszczyk, J. Gustafson, C. Kachulis, E. Kearns, J. L. Raaf, J. L. Stone, L. R. Sulak, S. Berkman, S. Tobayama, M. Goldhaber, M. Elnimr, W. R. Kropp, S. Mine, S. Locke, P. Weatherly, M. B. Smy, H. W. Sobel, V. Takhistov, K. S. Ganezer, J. Hill, J. Y. Kim, I. T. Lim, R. G. Park, A. Himmel, Z. Li, E. O'Sullivan, K. Scholberg, C. W. Walter, T. Ishizuka, T. Nakamura, J. S. Jang, K. Choi, J. G. Learned, S. Matsuno, S. N. Smith, J. Amey, R. P. Litchfield, W. Y. Ma, Y. Uchida, M. O. Wascko, S. Cao, M. Friend, T. Hasegawa, T. Ishida, T. Ishii, T. Kobayashi, T. Nakadaira, K. Nakamura, Y. Oyama, K. Sakashita, T. Sekiguchi, T. Tsukamoto, KE. Abe, M. Hasegawa, Y. Nakano, A. T. Suzuki, Y. Takeuchi, T. Yano, S. V. Cao, T. Hayashino, T. Hiraki, S. Hirota, K. Huang, M. Jiang, A. Minamino, KE. Nakamura, T. Nakaya, B. Quilain, N. D. Patel, R. A. Wendell, L. H. V. Anthony, N. McCauley, A. Pritchard, Y. Fukuda, Y. Itow, M. Murase, F. Muto, P. Mijakowski, K. Frankiewicz, C. K. Jung, X. Li, J. L. Palomino, G. Santucci, C. Vilela, M. J. Wilking, C. Yanagisawa, S. Ito, D. Fukuda, H. Ishino, A. Kibayashi, Y. Koshio, H. Nagata, M. Sakuda, C. Xu, Y. Kuno, D. Wark, F. Di Lodovico, B. Richards, R. Tacik, S. B. Kim, A. Cole, L. Thompson, H. Okazawa, Y. Choi, K. Ito, K. Nishijima, M. Koshiba, Y. Totsuka, Y. Suda, M. Yokoyama, R. G. Calland, M. Hartz, K. Martens, C. Simpson, Y. Suzuki, M. R. Vagins, D. Hamabe, M. Kuze, T. Yoshida, M. Ishitsuka, J. F. Martin, C. M. Nantais, H. A. Tanaka, A. Konaka, S. Chen, L. Wan, Y. Zhang, A. Minamino, and R. J. Wilkes
